Reachability analysis of first-order definable pushdown systems

We study pushdown systems where control states, stack alphabet, and transition relation, instead of being finite, are first-order definable in a fixed countably-infinite structure. We show that the reachability analysis can be addressed with the well-known saturation technique for the wide class of oligomorphic structures. Moreover, for the more restrictive homogeneous structures, we are able to give concrete complexity upper bounds. We show ample applicability of our technique by presenting several concrete examples of homogeneous structures, subsuming, with optimal complexity, known results from the literature. We show that infinitely many such examples of homogeneous structures can be obtained with the classical wreath product construction.

==> closure.tex <==

\section{Closure properties}

We study closure properties of context-free languages in sets with atoms.

Fix a logical structure $\atoms$, and let $A, B$ two orbit-finite FO-definable sets with atoms from $\atoms$.  
% and $\btoms$ be two logical structures. % over the same vocabulary.
A \emph{substitution $\sigma$ from $A$ to $B$} is a subset of $A\times B^*$.
%
A substitution $\sigma$ is \emph{context-free} when $\sigma$ is a context-free language over $A \cup B$.
%
A substitution $\sigma$ induces a function that maps from $A$ to languages over $B$
by defining $\sigma(a) = \setof {w \in B^*} {(a, w) \in \sigma}$,
which extends homomorphically to a function mapping from $A^*$ to languages over $B$
by $\sigma(\varepsilon) = \set \varepsilon$, and $\sigma(u_1 \cdot u_2) = \sigma(u_1) \cdot \sigma(u_2)$ when $u_1, u_2 \in A^*$,
where on the right we mean concatenation of languages.

\begin{lemma}
	\label{lem:substitution}
	Let $\sigma$ be a context-free substitution from $A$ to $B$,
	and let $L$ be a context-free language over $A$.
	Then, $\sigma(L)$ is a context-free language over $B$.
\end{lemma}
%
\noindent
Note that if $B$ is finite, then $\sigma(L)$ a language over a finite alphabet,
and thus a classical context-free language according to the lemma.
%
\begin{proof}
	%
	Let $\delta_0 \subseteq V \times (V \cup A)^*$ be a FO-definable set of productions,
	where $V$ are the non-terminal symbols,
	s.t. the context-free language $L$ is generated by the initial symbol $S_0 \in V$.
	%
	Let $\delta_1 \subseteq T \times (T \cup (A \cup B))^*$ be a FO-definable set of productions,
	where $T$ are the non-terminal symbols,
	and s.t. the context-free substitution $\sigma$ is generated by the initial symbol $S_1 \in T$.
	%
	We assume w.l.o.g. that $V$ and $T$ are disjoint.
	%	
	We construct a context-free grammar $\delta_2 \subseteq (V \cup T) \times (V \cup T \cup B)^*$
	with non-terminals in $V \cup T$ generating $\sigma(L)$ from $S_0$.
	%
	W.l.o.g. we assume that productions in $\delta_0$ and in $\delta_1$ are in Greibach normal form,
	and that $\delta_1$ does not have $\epsilon$-productions of the form $S_1 \goesto \varepsilon v$.
	%
	For each $X \goesto a u \in \delta_0$ with $a \in A$,
	and for each $S_1 \goesto a v \in \delta_1$,
	we add the production $X \goesto \varepsilon vu \in \delta_2$.
	%
	Clearly, $\delta_2$ is FO-definable by projecting away $a$.
	%
	TODO: give formal construction of the logical formula for $\delta_2$.
\end{proof}

\begin{corollary}
	Context-free languages are closed under union, concatenation, Kleene star, and homomorphism.
\end{corollary}

==> express.tex <==

% !TEX root = main.tex

\section{\Fodef prefix rewriting and context-free grammars}


We will use later the \emph{de-atomization} function 
\[
\biguplus_{l \in L} \  X_l \quad  \to \quad L
\] 
that maps $x \in X_l$ to $l$, for every $l \in L$.

Now we investigate how robust is the definition of pushdown automata with respect to other formulations, 
like prefix rewriting systems or context-free grammars. 
Classically,  prefix rewriting systems are equivalent to PDA up to isomorphism of transition graphs, while context-free grammars are
equivalent to PDA up to language generated, but not up to isomorphism of transition graphs.

A \emph{prefix-rewriting system} consists of a finite set $S$ of symbols, a finite alphabet $A$, and a set of rules
\[
\delta \subseteq S^{\leq m} \times A \times S^{\leq n}, \quad \text{ for some } m, n \in \nat.
\] 
In the classical version, PDA (with acceptance by empty stack) are exactly prefix-rewriting systems with left-hand sides
belonging to $S^{\leq 2}$.

Fix the atoms $\atoms$. We obtain the definition of \fodef (\qfdef) prefix rewriting system 
by relaxing finiteness of $S$ and $A$ to orbit-finiteness, and by additionally requiring $S$, $A$, and $\delta$ to be \fodef (\qfdef).
Similarly as before, in \emph{constraint} \fodef prefix rewriting system the set of left-hand sides of all the rules in $\delta$ is orbit-finite.

Clearly, \fodef prefix rewriting generalizes \fodef PDA.
We claim that the constraint prefix rewriting is not more powerful than constraint pushdown automata:
\begin{theorem}
Let $\atoms$ be an arbitrary relational structure. For every constrained prefix rewrite system $\cal P$ there is a constrained PDA $\autom$
such that the transition graphs generated by $\cal P$ and $\autom$ are related by an equivariant bijection. 
\end{theorem}

Now we define \fodef context-free grammars. As usual, we start with the classical definition: an alphabet $A$,
a set of nonterminals $V$, and a set of production rules
\[
\delta \subseteq V \times (V \cup A)^{\leq n}, \quad \text{ for some } n \in \nat.
\]
Along the same lines as before, we require $A$ and $V$ to be orbit-finite (but not necessarily $\delta$),
and moreover $A$, $V$ and $\delta$ to be \fodef. Note that there is no constraint version now, as the left-hand sides of rules
contain exactly one symbol. In fact, \fodef context-free grammars (CFG) are the same as \emph{stateless} \fodef PDA.

For a fair comparison of languages generated by context-free grammars and PDA,
assume from now on that the input alphabet of a PDA contains a distinguished symbol $\varepsilon$.
Thus the transition relation of a PDA is of the form:
\[
\delta \subseteq Q \times S \times (A \cup \{\varepsilon\}) \times Q \times S^{\leq n}, \quad \text{ for some } n \in \nat.
\] 
The language generated by a PDA is ...

The following fact is an easy exercise (see for instance~\cite{BKL14}, where this observation has been made for homogeneous atoms):
\begin{proposition}
For oligomorphic atoms $\atoms$, PDA and context-free grammars recognize the same languages.
\end{proposition}

Hence for oligomorphic atoms the picture is the same as classically.
On one side, all the three models define the same class of languages.
On the other hand, up to equivariant bijection there are two classes of transition graphs:
pushdown graphs and context-free graphs.

The picture is slightly more complex for non-oligomorphic atoms.
It is easily seen that pushdown languages are in general a strict superclass of context-free languages (we demonstrate this
for timed atoms in the next section). 

For future comparison with other models from literature, we distinguish two subclasses of \fodef PDA:
\fodef PDA with atomless control states, and \fodef PDA with atomless stack alphabet.
Both this subclasses are automatically constrained.
%
\begin{theorem}
Let $\atoms$ be an arbitrary logical structure. \Fodef PDA with atomless control states recognize the same languages as
context-free grammars.
\end{theorem}
%
Context-free languages satisfy the following pumping lemma....

Extend de-atomization function for an alphabet $A$ to words over $A$ (point-wise), and  to languages over $A$ (direct image).
Thus de-atomization of a language is a language over de-atomization of its alphabet, which is necessarily finite.
It is an easy observation that:
\begin{proposition}
De-atomizations of languages of \fodef PDA with atomless control states, as well as of \fodef PDA with atomless stack alphabet, 
are (classically) context-free.
\end{proposition}
In summary, we obtain the picture of language classes as in Fig.~\ref{fig:languages}.

\begin{figure}[htp] 
\label{fig:languages}
\centering{\includegraphics[scale=0.25]{languages.pdf}}
\caption{Classes of pushdown languages}
\end{figure}





==> fig_constraints.tex <==

\begin{figure}
	
	\begin{subfigure}[b]{\linewidth}
		\centering
		\begin{tikzpicture}[x=1.5cm]
	
			\draw[->,thick,>=latex] (0,0) -- (5,0) node [below right] {$\scriptstyle \text{time}$};
			%\draw[thick] (0,0) -- ++(0, 5pt);
			\draw[thick] (1,0) -- ++(0, 5pt) node [below = 1ex] {$\push\alpha$};
			\draw[thick] (2,0) -- ++(0, 5pt);
			\draw[thick] (4,0) -- ++(0, 5pt) node [below = 1ex] {$\begin{array}{cc}\text{corresponding} \\ \pop{\alpha \models \psi}\end{array}$};

			\fill([xshift=5pt]1,0.25) rectangle node[above] {$k$} ([xshift=-5pt]2,0.35); 
			\fill([xshift=5pt]2,0.25) rectangle node[above] {cannot reset $x$ here} ([xshift=-5pt]4,0.35);  
		
		\end{tikzpicture}
		
		\caption{Case $k\geq0$.}
		
	\end{subfigure}
	\\[4ex]
	\begin{subfigure}[b]{\linewidth}
		\centering
		\begin{tikzpicture}[x=1.5cm]
	
			\draw[->,thick,>=latex] (0,0) -- (5,0) node [below right] {$\scriptstyle \text{time}$};
			\draw[thick] (0,0) -- ++(0, 5pt);
			\draw[thick] (1,0) -- ++(0, 5pt) node [below = 1ex] {$\push\alpha$};
			%\draw[thick] (2,0) -- ++(0, 5pt);
			\draw[thick] (4,0) -- ++(0, 5pt) node [below = 1ex] {$\begin{array}{cc}\text{corresponding} \\ \pop{\alpha \models \psi}\end{array}$};

			\fill([xshift=5pt]0,0.25) rectangle node[above] {$-k$} ([xshift=-5pt]1,0.35); 
			\fill([xshift=5pt]0,0.85) rectangle node[above] {cannot reset $x$ here} ([xshift=-5pt]4,.95);  

		\end{tikzpicture}
		
		\caption{Case $k\leq0$.}
		
	\end{subfigure}
	
	\caption{Reset restriction on $x$ when $z - x \lesssim k \in \psi$.}
	\label{fig:reset_restriction}
	
\end{figure}

\begin{figure}
	
	\begin{subfigure}[b]{\linewidth}
		\centering	
		\begin{tikzpicture}[x=1.5cm]
	
			\draw[->,thick,>=latex] (0,0) -- (5,0) node [below right] {$\scriptstyle \text{time}$};
			%\draw[thick] (0,0) -- ++(0, 5pt);
			\draw[thick] (1,0) -- ++(0, 5pt) node [below = 1ex] {$\push\alpha$};
			\draw[thick] (2,0) -- ++(0, 5pt);
			\draw[thick] (4,0) -- ++(0, 5pt) node [below = 1ex] {$\begin{array}{cc}\text{corresponding} \\ \pop{\alpha \models \psi}\end{array}$};

			\fill([xshift=5pt]1,0.25) rectangle node[above] {$k$} ([xshift=-5pt]2,0.35); 
			\fill([xshift=5pt]2,0.25) rectangle node[above] {must reset $x$ here} ([xshift=-5pt]4,0.35);  
		
		\end{tikzpicture}
		
		\caption{Case $k\geq0$.}
		
	\end{subfigure}
	\\[4ex]
	\begin{subfigure}[b]{\linewidth}
		\centering
		\begin{tikzpicture}[x=1.5cm]
	
			\draw[->,thick,>=latex] (0,0) -- (5,0) node [below right] {$\scriptstyle \text{time}$};
			\draw[thick] (0,0) -- ++(0, 5pt);
			\draw[thick] (1,0) -- ++(0, 5pt) node [below = 1ex] {$\push\alpha$};
			%\draw[thick] (2,0) -- ++(0, 5pt);
			\draw[thick] (4,0) -- ++(0, 5pt) node [below = 1ex] {$\begin{array}{cc}\text{corresponding} \\ \pop{\alpha \models \psi}\end{array}$};

			\fill([xshift=5pt]0,0.25) rectangle node[above] {$-k$} ([xshift=-5pt]1,0.35); 
			\fill([xshift=5pt]0,0.85) rectangle node[above] {must reset $x$ here} ([xshift=-5pt]4,.95);  

		\end{tikzpicture}
		
		\caption{Case $k\leq0$.}
		
	\end{subfigure}
	
	\caption{Reset obligation on $x$ when $z - x \gtrsim k \in \psi$.}
	\label{fig:reset_obligation}
	
\end{figure}

\begin{figure}
	
%	\begin{subfigure}[b]{\linewidth}
%		\centering	
		\begin{tikzpicture}[x=1.5cm]
	
			\draw[->,thick,>=latex] (0,0) -- (5,0) node [below right] {$\scriptstyle \text{time}$};
			\draw[thick] (0,0) -- ++(0, 5pt) node [below = 1ex] {$\push\alpha$};
			%\draw[thick] (1,0) -- ++(0, 5pt) node [below = 1ex] {$\push\alpha$};
			\draw[thick] (2,0) -- ++(0, 5pt) node [below = 1ex] {next pop};
			\draw[thick] (4,0) -- ++(0, 5pt) node [below = 1ex] {$\begin{array}{cc}\text{corresponding} \\ \pop{\alpha \models \psi}\end{array}$};

			\fill([xshift=5pt]0,0.25) rectangle node[above] {$x$ reset either here} ([xshift=-5pt]2,0.35); 
			\fill([xshift=5pt]2,0.25) rectangle node[above] {or here} ([xshift=-5pt]4,0.35);  
		
		\end{tikzpicture}
		
%		\caption{Case $k\geq0$.}
		
%	\end{subfigure}

	\caption{Guess when $x$ is reset.}
	\label{fig:reset_obligation_guess}
	
\end{figure}

==> grammars.tex <==

% !TEX root = main.tex

\section{\Fodef context-free grammars}


Now we define \fodef context-free grammars. As usual, we start with the classical definition: an alphabet $A$,
a set of nonterminals $V$, and a set of production rules
\[
\delta \subseteq V \times (V \cup A)^{\leq n}, \quad \text{ for some } n \in \nat.
\]
Along the same lines as before, we require $A$ and $V$ to be orbit-finite (but not necessarily $\delta$),
and moreover $A$, $V$ and $\delta$ to be \fodef.  
In fact, \fodef context-free grammars (CFG) are \emph{stateless} \fodef PDA, where every transition pops exactly one
symbol from the stack.


The following fact is an easy exercise (see for instance~\cite{BKL14}, where this observation has been made for homogeneous atoms):
\begin{theorem}
For oligomorphic atoms $\atoms$, PDA and context-free grammars recognize the same languages.
\end{theorem}

Hence for oligomorphic atoms the picture is the same as classically.
On one side, all the three models define the same class of languages.
On the other hand, up to equivariant bijection there are two classes of transition graphs:
pushdown graphs and context-free graphs.



==> proofs.tex <==

% !TEX root = main.tex



\section{Complexity for homogeneous atoms (proof sketch)}
\label{sec:complexity proof}




==> removed.tex <==

\subsection{Configuration-to-configuration reachability}

\centerline{\textcolor{blue}{(SL: this subsection to be rewritten)}}

A standard decision problems is to decide, for two given configurations, if on of them is reachable from the other.
In the setting of \fodef automata we know that the reachability relation is equivariant, i.e., invariant under automorphisms,
hence it is reasonable to require equivariant subsets of initial and final configurations as input, instead of individual configurations.
We formulate the \emph{decision reachability problem} for regular subsets of configurations:
given \fodef PDA $\aaut$ and two \fodef NFA $\baut$ and $\caut$,
it asks if there are some configurations
\[
b \in L_{\aaut}(\baut) \text { and } c \in L_{\aaut}(\caut)  \text{ with } \transtrans{c}{}{b} \text{ ?}
\]


\begin{corollary} \label{cor:decision reachability}
Under the assumptions of Theorems~\ref{thm:pda decid oligo}, or Theorem~\ref{thm:pda decid homo},
the decision reachability problem has the same complexity as the inverse reachability problem.
\end{corollary}
%
Indeed, the decision reachability problem for $\aaut$, $\baut$ and $\caut$ is solved by:
first, computing an NFA $\baut'$ to describe the inverse reachability set $\invreach{\aaut}{L_{\aaut}(\baut)}$; and then
by testing the intersection of $\baut'$ and $\caut$ for non-emptiness.
Corollary~\ref{cor:decision reachability} follows from the effective closure of \fodef NDA under intersection,
and from decidability of non-emptiness of \fodef NFA. The details are omitted.
\slcomm{should details be discussed?}

%following empty-stack reachability problem which asks,
%for a PDA $\aaut'$, an atom-less stack symbol $\bot$ and an atom-less initial state $i$, 
%whether an empty-stack configuration is reachable from the initial configuration $(i, \bot)$:
%\[
%\transtrans{i, \bot}{}{q, \ew}, \quad \text{ for some state } q \text{ of } \aaut'.
%\] 
%The reduction, i.e., a transformation from $\aaut$ to $\aaut'$, amounts to wiring the sets $I$ and $F$ into $\aaut$. First, a non-deterministically chosen 
%element of $I$ is reached by $\aaut'$ before the actual execution of $\aaut$ starts. 
%Second, at any control state $\aaut'$ can non-deterministically start testing if the actual configuration belongs to $F$; 
%on a successful result of the test, the bottom stack symbol $\bot$ is removed.
%
%Finally, the empty-stack reachability problem is easily solvable by first computing an NFA $\baut'$ describing
%the inverse reachability set with respect to the set of empty-stack configurations, and then checking if $\baut'$ 
%contains a transition $\trans{i}{\bot}{f}$ for some state $q$ of $\aaut'$.

The upper bound of Corollary~\ref{cor:pda decid homo} matches the lower \exptime bound for reachability over
pushdown register automata~\cite{MRT14}. In case of equality atoms, our model subsumes the model of~\cite{MRT14},
which allows us to deduce from Corollaries~\ref{cor:pda decid homo} and~\ref{cor:decision reachability} the following:
\begin{corollary}
For a structure of atoms $\atoms$ satisfying assumptions of Corollary~\ref{cor:pda decid homo},
the decision reachability problem for \fodef PDA is
\begin{itemize}
\item \exptime-complete in general,
\item in polynomial time, for a fixed bound on dimension of input automata.
\end{itemize}
\end{corollary}


In the remainder of Section~\ref{sec:oligo} we briefly comment on relationship with automata in sets with atoms~\cite{},
and then sketch the proofs of Theorems~\ref{thm:pda decid oligo} and~\ref{thm:pda decid homo}.


\subsection{\Fodef sets vs sets with atoms}

Automata in sets with atoms (see~\cite{} for a thorough treatment of this topic) are obtained by
reinterpreting the classical definitions with finiteness replaced by orbit-finiteness.
When atoms are oligomorphic,
the setting of \fodef sets is a restriction of the general setting of sets with atoms~\cite{}.  
However in case of oligomorphic atoms the generality is not lost:

\begin{proposition} \label{fact:quotient}
Let $\atoms$ be a oligomorphic (homogeneous relational) structure. Then
for every orbit-finite equivariant set $Y$ there are \fodef (\qfdef) set $X$ and an \fodef (\qfdef) equivalence $\sim\ \subseteq X\times X$,
such that $Y$ is in equivariant bijection with $\quot{X}{\sim}$.
\end{proposition}
\slcomm{proof in app}

Thus an automaton (a PDA, NFA, or other) in sets with atoms is a quotient of its counterpart in \fodef sets,
by an \fodef equivalence. As the quotient preserves reachability in case of PDA,
we claim that all results stated above apply directly to the general setting of equivariant sets with atoms.


